A Control-Bounded Quadrature Leapfrog ADC

In this paper, the design flexibility of the control-bounded analog-to-digital converter principle is demonstrated. A band-pass analog-to-digital converter is considered as an application and case study. We show how a low-pass control-bounded analog-to-digital converter can be translated into a band-pass version where the guaranteed stability, converter bandwidth, and signal-to-noise ratio are preserved while the center frequency for conversion can be positioned freely. The proposed converter is validated with behavioral simulations on several filter orders, center frequencies, and oversampling ratios. Additionally, we consider an op-amp circuit realization where the effects of first-order op-amp non-idealities are shown. Finally, robustness against component variations is demonstrated by Monte Carlo simulations.

==> figures/02LP_LF.tex <==

\section{Old...}
The \ac{CBADC} concept, cf. \Eq{eq:ct_observation}, builds on the idea that an \ac{AS} stabilized by a \ac{DC} amounts to an implicit \ac{A/D} conversion.
As an example of such an \ac{AS}, consider the system within one of the dashed boxes in \Fig{fig:leapfrog-structure}.
This example shows a low-pass \ac{LF} \ac{AS} \cite{M:20}, parameterized by a forward and feedback gain $\beta$ and $\alpha$.
To turn the \ac{AS} into an \ac{ADC}, it's stabilized by a \ac{DC} through the control signals $s_1(t), \dots, s_N(t)$. A \ac{CBADC}'s overall conversion performance follows from the open-loop gain of the \ac{AS} in combination with a bounded state swing on the state variables $x_\ell(t)$ enforced by the \ac{DC}—particularly, a large \ac{AS} gain in combination with a, \ac{DC} enforced, small state swing result in good conversion performance.





In a subsequent step, the \ac{CBADC}'s final output follows from the control signals as % the discrete-time convolution of $N$ \ac{FIR} filters as
\begin{IEEEeqnarray}{rCl}
    \hat{u}[k]  & \eqdef & \sum_{\ell = 1}^N (h_\ell \ast s_\ell)[k]. \label{eq:estimate}
\end{IEEEeqnarray}
where the \ac{FIR} filter coefficients $h_1[.], \dots, h_\ell[.]$, in \Eq{eq:estimate}, depend on the parametrization of the \ac{AF}, i.e., the combined \ac{AS} and \ac{DC}. Furthermore, the discrete time control signals in \Eq{eq:estimate} are
related to their continuous time counterparts as 
\begin{IEEEeqnarray}{rCl}
    s_\ell(t) & = & \sum_k s_\ell[k] \theta_\ell(t - kT)
\end{IEEEeqnarray}
where the \ac{DC} updates the control signals with a clock frequency of $f_s\eqdef1/T$ and $\theta(t)$ is the corresponding \ac{DAC}  waveform.
The FIR filters $h_1[.],\dots,h_N[.]$ in \Eq{eq:estimate} can be calculated analytically as in \cite{MWL:21} or via calibration as in \cite{MMBFL:22}. Beware that component variation in the \ac{AS} or \ac{DC} will introduce a significant estimation error if not accounted for in $h_1[.],\dots,h_N[.]$, cf. \cite{FMWLY:2022} and \cite{MMBFL:22}. 

The \ac{AS} is conveniently described using state-space equations;
an $N$th order \ac{LF} \ac{AS}, follows from the differential equations
\begin{IEEEeqnarray}{rCl}
    \dot{\vct{x}}(t) & = & \mat{A}_{\text{LF}} \vct{x}(t) + \mat{B}_{\text{LF}} u(t) + \vct{s}(t) \label{eq:state_equations_leapfrog} %\\
\end{IEEEeqnarray}
where
\begin{IEEEeqnarray}{rCl}
    \vct{x}(t) &\eqdef& \begin{pmatrix}x_1(t), \dots, x_N(t)\end{pmatrix}^\T, \\
    \vct{s}(t) &\eqdef& \begin{pmatrix}s_1(t), \dots, s_N(t)\end{pmatrix}^\T, \\
    \mat{A}_{\text{LF}} & \eqdef &
    \begin{pmatrix}
        0 & \alpha \\
        \beta & 0 & \ddots \\ 
         & \ddots & \ddots & \alpha \\
         &  & \beta & 0  \\
    \end{pmatrix} \in \R^{N \times N},
\end{IEEEeqnarray}
and $\mat{B}_{\text{LF}} \eqdef \begin{pmatrix}\beta, 0,\dots, 0\end{pmatrix}^\T\in \R^N$.

The \ac{LF}'s homogeneous and modular structure enables design equations where %, based on closed form design equations for the parameters $\beta, \alpha$ and $\kappa$ 
for a given $N$, $\wb$, and \ac{OSR},% i.e., $\text{\ac{OSR}} \eqdef \frac{\pi f_s}{\omega_{\mathcal{B}}}$,
\begin{IEEEeqnarray}{rCl}%
\text{SNR} & \propto & \left(\text{OSR}\right)^{2N} \labell{eq:SNR_scaling} 
\end{IEEEeqnarray}
and stability %and the converters's bandwidth 
follow from the relations
\begin{IEEEeqnarray}{rCl}
    |\beta| & = & \frac{\wb \cdot \text{OSR}}{2 \pi} \labell{eq:stability} \\
    \kappa & = & -\beta = \frac{\wb^2}{4\alpha} \labell{eq:leapfrog_relation}
\end{IEEEeqnarray}
where 
$\wb$ [rad/s] is the targeted angular signal bandwidth.
\cite{FMWLY:2022} showed that the nominal performance of a low-pass \ac{LF} \ac{CBADC} is similar to that of a heuristically optimized \ac{CTSDM} with the same loop filter order $N$, fixed \ac{OSR}, and the same number of quantization levels. 
















































\begin{figure*}[tbp]
    \begin{center}
        \resizebox{\textwidth}{!}{
            \input{figures/leapfrog-structure}
        }
        \caption{\label{fig:leapfrog-structure} The quadrature Leapfrog analog system which is is the combination of two Leapfrog structures, as in \Sec{sec:leapfrog},
        connected by the $\omega_n$ paths. The system is stabilized via the control signals $s_1(t),\dots,s_N(t),\bar{s}_1(t),\dots,\bar{s}_N(t)$ resulting from $N$ quadrature local digital controls as shown in \Fig{fig:digital_control_zero_order_hold}.
        }
    \end{center}
\end{figure*}






















==> figures/op-amp_model.tex <==
\begin{circuitikz}[european voltages]

\node[rground] (ground) at (0,0) {};
\node[buffer] (buffer) at ($(ground) + (3.75, 1.5)$) {1};

\draw (ground)
    to[cvsource,l=$g_m \cdot v_{\mathrm{in}}(t)$] ++(0,1.5)
    to[short,-*] ++(1.125,0) coordinate (R) {}
    to[short,-*] ++(1.125,0) coordinate (C) {}
    to[short] (buffer.in)
    (buffer.out) to[short,-o] ++(0,0)
;

\node[right] at (buffer.out) {$v_{\mathrm{out}}(t)$};

\draw (R) to[R,l=$R$] ++(0,-1.5)
    coordinate (R_ground) {}
    to[short,-*] (ground);

\draw (C) to[C,l=$C$] ++(0,-1.5)
    to[short,-*] (R_ground);

\end{circuitikz}

